Profound optical flares from the relativistic jets of active galactic nuclei

Intense outbursts in blazars are among the most extreme phenomena seen in extragalactic objects. Studying these events can offer important information about the energetic physical processes taking place within the innermost regions of blazars, which are beyond the resolution of current instruments. This work presents some of the largest and most rapid flares detected in the optical band from the sources 3C 279, OJ 49, S4 0954+658, Ton 599, and PG 1553+113, which are mostly TeV blazars. The source flux increased by nearly ten times within a few weeks, indicating the violent nature of these events. Such energetic events might originate from magnetohydrodynamical instabilities near the base of the jets, triggered by processes modulated by the magnetic field of the accretion disc. We explain the emergence of flares owing to the injection of high-energy particles by the shock wave passing along the relativistic jets. Alternatively, the flares may have also arisen due to geometrical effects related to the jets. We discuss both source-intrinsic and source-extrinsic scenarios as possible explanations for the observed large amplitude flux changes.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

